Non-formality of Voronov's Swiss-Cheese operads

The Swiss-Cheese operads, which encode actions of algebras over the little $n$-cubes operad on algebras over the little $(n-1)$-cubes operad, comes in several variants. We prove that the variant in which open operations must have at least one open input is not formal in characteristic zero. This is slightly stronger than earlier results of Livernet and Willwacher. The obstruction to formality that we find lies in arity $(2, 2^n)$, rather than $(2, 0)$ (Livernet) or $(4, 0)$ (Willwacher).

==> removed.tex <==
\section{Singular chain complexes and particular elements}

I think we should choose the $N$-dimensional euclidean space spanned by:
$$\{\vec e_0, \vec e_1, \dots, \vec e_{N-1}\}.$$

Let $\S^0:=\{-, +\}$, $\underline{N-1} := \{1, \dots, N-1\}$ and let $\vec b_{\epsilon i}:=\epsilon\vec e_i$ where $\epsilon \in \{-, +\}$.

Consider $A_N := \S^0\times\underline{N-1}$ with all elements open. We equip it with the $\mathbb Z_{2N-2}$-action that ``rotates by a quarter turn'', i.e., it is generated by:
\begin{align*}
  \epsilon i\cdot 1:=\begin{cases}
                       \epsilon(i+1), & \text{if } 1\leq i\leq N-2; \\
                       -\epsilon 1,   & \text{if } i=N-1.
                     \end{cases}
\end{align*}
This action is regular (i.e., free and transitive), so that for all $\epsilon i, \epsilon'i'\in A$ there is a unique element $\epsilon' i'-\epsilon i\in\mathbb Z_{2N-2}$ such that $\epsilon i\cdot (\epsilon' i'-\epsilon i)=\epsilon'i'$. Note that $\epsilon i\cdot (N-1)=-\epsilon i$.

We are going to define several elements of $\SCv_N$.
Recall from Definition~\ref{def:scv} that an element $x \in \SCv_N(A)$ (where $A$ is some bicolored set) by its components $x_a \in D^N \times [0, 1]$ for $a \in A$, where the first coordinate of $x_a$ represents the center of a little (half-)disk and the second coordinate represents its radius.
Let us first define the element $a \in \SCv_N(\{\colc, \colo\})$ by:
$$
  a_\colc:= \Bigl(\frac{3}{4}\vec e_0, \frac{1}{4} \Bigr),
  \quad
  a_\colo := \Bigl( \vec 0, \frac{1}{2} \Bigr),
$$
i.e., we consider a half-disk of radius $1/4$ centered at the origin and a little disk of radius $1/4$ centered $3/4$ units above the origin.
Next, we define the element $m \in \SCv_N(A_N)$ by:
$$
  m_{\epsilon i} := \Bigl( \frac{3}{4}\vec b_{\epsilon i}, \frac{1}{4}\Bigr),
$$
i.e., we consider a configuration of $N-1$ pairs of half-disks, one for each coordinate axis of $\{0\} \times \R^{N-1}$, centered on both sides of the origin.
Finally, we define the $(N-1)$-chain $l : \mathbb{S}^{N-1} \to \D_N(\mathbb{S}^0)$ by:
$$
  l_\epsilon(\vec x) := \bigl(\epsilon\frac{1}{2}\vec x, \frac{1}{2}\bigr), \qquad \forall \vec x \in \mathbb{S}^{N-1}.
$$

Let $A^+:=\{ \mathfrak c \}\sqcup A$. For each $\langle \epsilon_i\rangle\in \Pi_{\underline{N-1}}\S^0$ let
\begin{gather*}
  \beta^{\langle \epsilon_i\rangle}\in C_{N-1}\SC_NA^+\\
  \beta^{\langle \epsilon_i\rangle}_{ \mathfrak c }\vec t:=
  \left(
  \frac{3}{4}
  \left(
    \frac{1+3t_0}{4}\vec e_0
    +
    \sum_{j=1}^{N-1}t_j\vec b_{\epsilon_i i}
    \right)
  , \frac{1}{4(4-3t_0)}\right)\\
  \beta^{\langle\epsilon_i\rangle}_{\epsilon ' i' }\vec t
  :=\begin{cases}\left(\frac{3}{4+4t_0}\vec b_{\epsilon 'i'} , \frac{1}{(1+t_{i'})(4+4t_{0})}\right),
     & \epsilon' =\epsilon_{i'}    \\
    \left(\frac{3}{4+4t_0}\vec b_{\epsilon' i'} , \frac{1}{4+4t_{0}}\right),
     & \epsilon'\neq \epsilon_{i'}
  \end{cases}
\end{gather*}


\begin{figure}
  \centering
  \begin{tikzpicture}
    \node at (0, 2.9) {\includegraphics[scale=0.125]{BetaSC100.png}};
    \node at (-3.25, -1.5) {\includegraphics[scale=0.125]{BetaSC010.png}};
    \node at (3.25, -1.5) {\includegraphics[scale=0.125]{BetaSC001.png}};
    \node at (0, 0) {\includegraphics[scale=0.125]{BetaSC1:2.png}};
    \draw[thick, ->] (-0.1, 1.6)--(-1.9, -0.9);
    \draw[thick, ->] (-1.8, -1)--(1.8, -1);
    \draw[thick, ->] (0.1, 1.6)--(1.9, -0.9);

    \node at (0, 1.8) {\footnotesize$\vec e_0$};
    \node at (-1.95, -1.05) {\footnotesize$\vec e_1$};
    \node at (1.95, -1.05) {\footnotesize$\vec e_2$};
  \end{tikzpicture}
  \caption{$\beta^{++}$ for $N=3$.}
  \label{fig:my_label}
\end{figure}

\renato*{The figure is just a suggestion. We can alter it if you have any ideas on how to improve the illustration.
  If you want to mess around with the geogebra code I made a link:
  \url{https://www.geogebra.org/classic/p67vekna}}
\najib*{The figure is good! Just a little remark, the blue spheres are not of the same size in the middle figure, is it okay?}



Defining
\begin{align*}
  \eta & :=\sum_{\Pi_{\underline{N-1}}\S^0}
  \left(\prod_{\underline{N-1}}\epsilon_i\right)
  \left(a \circ_{\mathfrak o}\beta^{\langle\epsilon_i\rangle}
  +\beta^{\langle\epsilon_i\rangle}\circ_{-\epsilon_{N-1} (N-1)}a\right)
\end{align*}

I think we can build a homotopy between $l$ and $\eta+\eta\cdot(1_{\mathfrak c} 2_{\mathfrak c})$.

Pretty sure this is equivalent to the case $N=2$ in my thesis.

\renato*{Here I am writing an alternative set of cells that I think might work better. Instead of $m$ being a configuration of $2(N-1)$ half disks I think we can use just $N$. Not only there are fewer things moving, now there is only one possible choice of where one of the closed little disks is staying when the other is moving}

\najib{This looks promising! One thing that I hoped to achieve is to write some kind of inductive formula ; the $\beta$ in dimension $N+1$ should be obtained from the one in dimension $N$ glued nicely, but I didn't really manage to complete it.}

Let $\underline{N-1}_*=\{0, 1, \dots N-1\}$, $\vec b_0=\vec 0$ and $\vec b_i=\vec e_i$ for $i\in\underline{N-1}$.

Let $m\in\mathcal{SC}_N^{\text{vor}}(\underline{N-1}_*)$ be defined by:
$$
  m_i=\left(\frac{2}{3}\vec b_i, \frac{1}{3}\right)
$$
For each $i\in\underline{N-1}_*$ let $\beta^i\in \mathcal{SC}_N^{\text{vor}}(\{\mathfrak c\}\sqcup \underline{N-1}_*)$ be defined by
\begin{gather*}
  \beta^i_{\mathfrak c }\vec t:=
  \left(
  \frac{1+2t_0}{4}\vec e_0
  +
  \frac{2}{3}\left(\sum_{j=1}^{N-1}t_j\vec b_{j+i-1}\right)
  , \frac{1}{4(3-2t_0)}\right)\\
  \beta^i_j\vec t
  :=\begin{cases}\left(\frac{2-t_0}{3}\vec b_j , \frac{2-t_0}{(1+t_{j-i+1})6}\right),
     & j\neq i-1 \\
    \left(\frac{2-t_0}{3}\vec b_j , \frac{2-t_0}{6}\right),
     & j= i-1
  \end{cases}
\end{gather*}

\renato*[caption=Easier to generalize]{For $N=2$ the cycle homologous to $a\circ_{\mathfrak c}l$ is
  \begin{gather*}
    a\circ_{\mathfrak o}\beta^0+\beta^1\circ_0 a-(\beta^0\circ_1a+a\circ_{\mathfrak o}\beta^1)\cdot(1_{\mathfrak c}2_{\mathfrak c})\\
    +(a\circ_{\mathfrak o}\beta^0+\beta^1\circ_0 a)\cdot(1_{\mathfrak c}2_{\mathfrak c})-(\beta^0\circ_1a+a\circ_{\mathfrak o}\beta^1)
  \end{gather*}
  We can define
  \begin{align*}
    \eta:= & a\circ_{\mathfrak o}\beta^0    -a\circ_{\mathfrak o}\beta^1 \\
           & -\beta^0\circ_1a+\beta^1\circ_0a
  \end{align*}
  so that the above cycle is
  $$
    \eta+\eta\cdot (1_{\mathfrak c}2_{\mathfrak c})
  $$
  This isn't exactly what I did in my thesis, but I think this will be easier to generalise
}

Let
$$
  \eta:=\sum_{j=0}^{N-1} (-1)^{j(N-1)}(a\circ_{\mathfrak o}\beta^j-\beta^j\circ_{j-1}a)
$$
\renato*{
  I'm not 100\% sure about the signs. And I think $\partial(\eta +\eta\cdot(1_{\mathfrak c}2_{\mathfrak c}))$ isn't going to be exactly 0 when $N>2$. Might need some fixing}

For $0<i< N-1$ and $0\leq j\leq N-1$ we have by construction that
$$
  \partial_i\beta^j=\partial_{i+1}\beta^{j+1}
$$
and
$$
  \partial_{N-1}\beta^j=\partial_1\beta^{j-1}
$$
which implies

\begin{align*}
  \partial \eta & =\sum_{i=0}^{N-1}(-1)^i\partial_i\eta                                                                                 \\
                & = \sum_{i=0}^{N-1}(-1)^i\partial_i\left(
  \sum_{j=0}^{N-1} (-1)^{j(N-1)}(a\circ_{\mathfrak o}\beta^j-\beta^j\circ_{j-1}a)\right)                                                \\
                & =\sum_{i=0}^{N-1}\sum_{j=0}^{N-1}(-1)^{i+j(N-1)}(a\circ_{\mathfrak o}\partial_i\beta^j-\partial_i\beta^j\circ_{j-1}a) \\
                & =\left(\sum_{i=0}^{N-1}\sum_{j=0}^{N-1}(-1)^{i+j(N-1)}a\circ_{\mathfrak o}\partial_i\beta^j\right)
  -\left(\sum_{i=0}^{N-1}\sum_{j=0}^{N-1}(-1)^{i+j(N-1)}\partial_i\beta^j\circ_{j-1}a\right)                                            \\
                & =\left(\sum_{j=0}^{N-1}(-1)^{i+j(N-1)}a\circ_{\mathfrak o}\partial_0\beta^j\right)
  -\left(\sum_{i=0}^{N-1}\sum_{j=0}^{N-1}(-1)^{i+j(N-1)}\partial_i\beta^j\circ_{j-1}a\right)
\end{align*}


\renato*{Started a draft of the calculations. Not much so far}

% \section{General approach to non-formality}

% \najib*{Here we can explain how non-formality can be deduced from finding chains that bound cycles and produce non-trivial homology classes when composed.}

